Post-hoc Calibration of Neural Networks by g-Layers

Calibration of neural networks is a critical aspect to consider when incorporating machine learning models in real-world decision-making systems where the confidence of decisions are equally important as the decisions themselves. In recent years, there is a surge of research on neural network calibration and the majority of the works can be categorized into post-hoc calibration methods, defined as methods that learn an additional function to calibrate an already trained base network. In this work, we intend to understand the post-hoc calibration methods from a theoretical point of view. Especially, it is known that minimizing Negative Log-Likelihood (NLL) will lead to a calibrated network on the training set if the global optimum is attained (Bishop, 1994). Nevertheless, it is not clear learning an additional function in a post-hoc manner would lead to calibration in the theoretical sense. To this end, we prove that even though the base network ($f$) does not lead to the global optimum of NLL, by adding additional layers ($g$) and minimizing NLL by optimizing the parameters of $g$ one can obtain a calibrated network $g \circ f$. This not only provides a less stringent condition to obtain a calibrated network but also provides a theoretical justification of post-hoc calibration methods. Our experiments on various image classification benchmarks confirm the theory.

==> newcommands.tex <==
\newcommand{\IO}{{[ \m I \mid \vs 0 ]}}
\newcommand{\Rc}{{[ \m R \mid -\m R \dH C ]}}
\newcommand{\alg} {{\mbox{\rm\small alg}}}
\newcommand{\sym} {{\mbox{\rm\small sym}}}
\newcommand{\barH}{{\bar{\m H}}}
\newcommand{\barN}{{\bar{\vs N}}}
\newcommand{\barX}{{\bar{\vs X}}}
\newcommand{\barh}{{\bar{\v h}}}
\newcommand{\barm}{{\bar{\v m}}}
\newcommand{\barp}{{\bar{\v p}}}
\newcommand{\barv}{{\bar{\v v}}}
\newcommand{\barx}{{\bar{\v x}}}
\newcommand{\cam}{{\mbox{\rm\small cam}}}
\newcommand{\dH}[1]{{\tilde{\vs #1}}}
\newcommand{\depth}{\mbox{\rm depth}}
\newcommand{\Dh}[1]{{\tilde{\v #1}}}
\newcommand{\geom}{{\mbox{\rm\small geom}}}
\newcommand{\mah}{{\mbox{\rm\small Mah}}}
\newcommand{\hath}{{\hat{\v h}}}
\newcommand{\hatf}{{\hat{\v f}}}
\newcommand{\hatH}{{\widehat{\m H}}}
\newcommand{\hatA}{{\widehat{\m A}}}
\newcommand{\hatN}{{\hat{\vs N}}}
\newcommand{\hatX}{{\widehat{\vs X}}}
\newcommand{\hatm}{{\hat{\v m}}}
\newcommand{\hatp}{{\hat{\v p}}}
\newcommand{\hatu}{{\hat{\v u}}}
\newcommand{\hatx}{{\hat{\v x}}}
\newcommand{\haty}{{\hat{\v y}}}
\newcommand{\hatvP}{{\widehat{\vs P}}}
\newcommand{\hatP}{{\widehat{\m P}}}
\newcommand{\hatF}{{\widehat{\m F}}}
\newcommand{\lin}[2]{<#1; #2>}
\newcommand{\matxs}[1]{{\tt  \tilde{#1}}}
\newcommand{\pqrs}{^{pqrs}}
\newcommand{\tens}[2]{#1_{#2}}
\newcommand{\tilA}{{\widetilde{\m A}}}
\newcommand{\tilC}{{\widetilde{\vs C}}}
\newcommand{\tilH}{{\widetilde{\m H}}}
\newcommand{\tilx}{{\tilde{\v x}}}
\newcommand{\tilh}{{\tilde{\v h}}}
\newcommand{\x}{{\mbox{\sl\sc x}}}
\newcommand{\y}{{\mbox{\sl\sc y}}}
\newcommand{\z}{{\mbox{\sl\sc z}}}
\newcommand{\T}{{\mbox{\sl\sc t}}}
\newcommand{\X}{{\mbox{\sl\sc x}}}
\newcommand{\Y}{{\mbox{\sl\sc y}}}
\newcommand{\Z}{{\mbox{\sl\sc z}}}
\newcommand{\W}{{\mbox{\sl\sc w}}}
%
% for subscripts/superscripts for affine and projective H's etc
%
\newcommand{\HE}{{\rm E}}
\newcommand{\HM}{{\rm M}}
\newcommand{\HS}{{\rm S}}
\newcommand{\HA}{{\rm A}}
\newcommand{\HP}{{\rm P}}

% \newcommand{\symm}{{\mbox{\small S}}}
% \newcommand{\anti}{{\mbox{\small A}}}
% would prefer to have these symbols with small upper case
% but caption lines then too long
\newcommand{\symm}{{\mbox{\tt s}}}
\newcommand{\anti}{{\mbox{\tt a}}}
\newcommand{\ray}[2]{\overline{#1 #2}}

% The calibration matrix -- Andrew, we can not use $\m C$, since
% this is used (in close proximity) as the symbol for a conic.
\newcommand{\K}{\m K}

% Temporarily like this to satisfy version of latex
%\newcommand{\x}{X}
%\newcommand{\y}{Y}
%\newcommand{\z}{Z}
%\newcommand{\T}{T}
%\newcommand{\X}{X}
%\newcommand{\Y}{Y}
%\newcommand{\Z}{Z}
%\newcommand{\W}{W}

% For the image of X under the Carlsson map
\newcommand{\invX}{{\bar{\vs X}}}
\newcommand{\barC}{{\bar{\vs C}}}
\newcommand{\invC}{{\bar{\vs C}}}
\newcommand{\barQ}{{\bar{\m Q}}}
\newcommand{\barP}{{\bar{\m P}}}
\newcommand{\barF}{{\bar{\m F}}}


==> tables/ECE.tex <==
\begin{table*}[t]
\scriptsize
\centering
\begin{tabular}{ll|cccccc}
\toprule
Dataset                    & Model          & Uncalibrated & Temp. Scaling & Vector Scaling & MS-ODIR & Dir-ODIR & \textbf{$g$-layer} \\ \midrule
\multirow{5}{*}{CIFAR-10}  & Resnet-110     & 4.750      & 1.132       & 1.084        & 1.052 & 1.144  & \textbf{0.509}          \\
                           & Resnet-110-SD  & 4.113      & \textbf{0.555}       & 0.733        & 0.599 & 0.739  & 0.694             \\
                           & DenseNet-40    & 5.500      & \textbf{0.946}       & 1.115        & 1.006 & 1.095  & 1.065             \\
                           & Wide Resnet-32 & 4.505      & \textbf{0.784}       & 0.857        & \textbf{0.784} & 0.796  &             0.978\\
                           \midrule
                        %   & Lenet-5        & 0.05180      & 0.01665       & 0.01419        & 0.01442 & 0.01265  & \textbf{0.02122}             \\ \midrule
% \multirow{5}{*}{CIFAR-100} & Resnet-110     & 0.18481      & 0.02380       & 0.02656        & 0.02718 & 0.02896  & ?             \\
%                           & Resnet-110-SD  & 0.15861      & 0.01214       & 0.01690        & 0.02203 & 0.02047  & ?             \\
%                           & DenseNet-40    & 0.21156      & 0.00902       & 0.01338        & 0.02709 & 0.00962  & ?             \\
%                           & Wide Resnet-32 & 0.18784      & 0.01472       & 0.01665        & 0.02821 & 0.01991  & ?             \\
%                           & Lenet-5        & 0.12125      & 0.01499       & 0.01244        & 0.01383 & 0.01998  & ?             \\ \midrule
% \multirow{2}{*}{ImageNet}  & Densenet-161   & 0.05720      & 0.01942       & 0.02583        & 0.04333 & 0.03926  & ?             \\
%                           & Resnet-152     & 0.06543      & 0.02078       & 0.02642        & 0.05353 & 0.04491  & ?             \\ \midrule
SVHN                       & Resnet-152-SD  & 0.862      & 0.607       & 0.612        & 0.616 & 0.590  & \textbf{0.359}      \\ \bottomrule      
\end{tabular}
%     \vspace{1ex}

\caption{\em ECE (Expected Calibration Error) comparisons against state of the art post-hoc calibration methods on image classification datasets: CIFAR-10 and SVHN, using various network architectures.}
\end{table*}

==> tables/PKSE.tex <==
\SKIP{
\begin{table}[]
\scriptsize
\begin{tabular}{ll|cccccc}
\toprule
Dataset &
  Model &
  Uncalibrated &
  Temp. Scaling &
  Vector Scaling &
  MS-ODIR &
  Dir-ODIR &
  \textbf{$g$-layer} \\ \midrule
\multirow{5}{*}{CIFAR-10} &
  Resnet-110 &
  0.04750 &
  0.00916 &
  0.00996 &
  0.00977 &
  0.01060 &
  \textbf{0.00305} \\
 &
  Resnet-110-SD &
  0.04102 &
  0.00362 &
  0.00430 &
  0.00358 &
  0.00389 &
  \textbf{0.00279} \\
  &
  DenseNet-40 &
  0.05493 &
  0.00900 &
  0.00890 &
  0.00897 &
  0.01057 &
  \textbf{0.00688} \\
 &
  Wide Resnet-32 &
  0.04475 &
  0.00296 &
  \textbf{0.00267} &
  0.00305 &
  0.00291 &
  0.00419 \\
%  &
%   Lenet-5 &
%   0.05038 &
%   0.00799 &
%   0.00839 &
%   0.00646 &
%   0.00854 &
%   0.02142 \\ \midrule
% \multirow{5}{*}{CIFAR-100} &
%   Resnet-110 &
%   0.18481 &
%   0.01489 &
%   0.01827 &
%   0.02845 &
%   0.02575 &
%   0.07704 \\
%  &
%   Resnet-110-SD &
%   0.15832 &
%   \textbf{0.00748} &
%   0.01303 &
%   0.03572 &
%   0.01645 &
%   0.09390 \\
%  &
%   DenseNet-40 &
%   0.21156 &
%   \textbf{0.00304} &
%   0.00483 &
%   0.02350 &
%   0.00618 &
%   0.12670 \\
%  &
%   Wide Resnet-32 &
%   0.18784 &
%   \textbf{0.01130} &
%   0.01642 &
%   0.02524 &
%   0.01788 &
%   0.08086 \\
%  &
%   Lenet-5 &
%   0.12117 &
%   0.01215 &
%   0.00768 &
%   0.01047 &
%   0.02125 &
%   0.06303 \\
% \midrule
% \multirow{2}{*}{ImageNet} &
%   Densenet-161 &
%   0.05721 &
%   0.00744 &
%   0.02014 &
%   0.04723 &
%   0.03103 &
%   0.06575 \\
%  &
%   Resnet-152 &
%   0.06544 &
%   0.00791 &
%   0.01985 &
%   0.05805 &
%   0.03528 &
%   0.04977 \\
\midrule
SVHN &
  Resnet-152-SD &
  0.00852 &
  0.00552 &
  0.00570 &
  0.00573 &
  0.00607 &
  \textbf{0.00265} \\
\bottomrule
\end{tabular}
    \vspace{1ex}

    \caption{\em KS calibration error~\cite{gupta-spline-iclr21} (in \%) comparisons against state-of-the-art post-hoc calibration methods on image classification datasets: CIFAR-10 and SVHN, using various network architectures.}
    \label{tab:res_PKSE}  
\end{table}
}

\SKIP{
% \begin{table}[]
% \scriptsize
\begin{tabular}{ll|cccccc}
\toprule
Dataset &
  Model &
  Uncalibrated &
  Temp. Scaling &
  Vector Scaling &
  MS-ODIR &
  Dir-ODIR &
  \textbf{$g$-layer} \\ \midrule
\multirow{5}{*}{CIFAR-10} &
  Resnet-110 &
  4.750 &
  0.916 &
  0.996 &
  0.977 &
  1.060 &
  \textbf{0.305} \\
 &
  Resnet-110-SD &
  4.102 &
  0.362 &
  0.430 &
  0.358 &
  0.389 &
  \textbf{0.279} \\
  &
  DenseNet-40 &
  5.493 &
  0.900 &
  0.890 &
  0.897 &
  1.057 &
  \textbf{0.688} \\
 &
  Wide Resnet-32 &
  4.475 &
  0.296 &
  \textbf{0.267} &
  0.305 &
  0.291 &
  0.419 \\
%  &
%   Lenet-5 &
%   5.038 &
%   0.799 &
%   0.839 &
%   0.646 &
%   0.854 &
%   2.142 \\ \midrule
% \multirow{5}{*}{CIFAR-100} &
%   Resnet-110 &
%   18.481 &
%   1.489 &
%   1.827 &
%   2.845 &
%   2.575 &
%   7.704 \\
%  &
%   Resnet-110-SD &
%   15.832 &
%   \textbf{0.748} &
%   1.303 &
%   3.572 &
%   1.645 &
%   9.390 \\
%  &
%   DenseNet-40 &
%   21.156 &
%   \textbf{0.304} &
%   0.483 &
%   2.350 &
%   0.618 &
%   12.670 \\
%  &
%   Wide Resnet-32 &
%   18.784 &
%   \textbf{1.130} &
%   1.642 &
%   2.524 &
%   1.788 &
%   8.086 \\
%  &
%   Lenet-5 &
%   12.117 &
%   1.215 &
%   0.768 &
%   1.047 &
%   2.125 &
%   6.303 \\
% \midrule
% \multirow{2}{*}{ImageNet} &
%   Densenet-161 &
%   5.721 &
%   0.744 &
%   2.014 &
%   4.723 &
%   3.103 &
%   6.575 \\
%  &
%   Resnet-152 &
%   6.544 &
%   0.791 &
%   1.985 &
%   5.805 &
%   3.528 &
%   4.977 \\
\midrule
SVHN &
  Resnet-152-SD &
  0.852 &
  0.552 &
  0.570 &
  0.573 &
  0.607 &
  \textbf{0.265} \\
\bottomrule
\end{tabular}
%     \vspace{1ex}

%     \caption{\em KS calibration error \cite{gupta-spline-iclr21} (in \%) comparisons against state of the art post-hoc calibration methods on image classification datasets: CIFAR-10 and SVHN, using various network architectures.}
%     \label{tab:res_PKSE}
% \end{table}
}



\begin{table*}[]
\scriptsize
\centering
\begin{tabular}{ll|cccccc}
\toprule
Dataset &
  Model &
  Uncalibrated &
  Temp. Scaling &
  Vector Scaling &
  MS-ODIR &
  Dir-ODIR &
  \textbf{$g$-layer} \\ \midrule
\multirow{5}{*}{CIFAR-10} &
  Resnet-110 &
  4.750 &
  0.916 &
  0.996 &
  0.977 &
  1.060 &
  \textbf{0.305} \\
 &
  Resnet-110-SD &
  4.102 &
  0.362 &
  0.430 &
  0.358 &
  0.389 &
  \textbf{0.279} \\
  &
  DenseNet-40 &
  5.493 &
  0.900 &
  0.890 &
  0.897 &
  1.057 &
  \textbf{0.688} \\
 &
  Wide Resnet-32 &
  4.475 &
  0.296 &
  \textbf{0.267} &
  0.305 &
  0.291 &
  0.419 \\
%  &
%   Lenet-5 &
%   5.038 &
%   0.799 &
%   0.839 &
%   0.646 &
%   0.854 &
%   2.142 \\ \midrule
% \multirow{5}{*}{CIFAR-100} &
%   Resnet-110 &
%   18.481 &
%   1.489 &
%   1.827 &
%   2.845 &
%   2.575 &
%   7.704 \\
%  &
%   Resnet-110-SD &
%   15.832 &
%   \textbf{0.748} &
%   1.303 &
%   3.572 &
%   1.645 &
%   9.390 \\
%  &
%   DenseNet-40 &
%   21.156 &
%   \textbf{0.304} &
%   0.483 &
%   2.350 &
%   0.618 &
%   12.670 \\
%  &
%   Wide Resnet-32 &
%   18.784 &
%   \textbf{1.130} &
%   1.642 &
%   2.524 &
%   1.788 &
%   8.086 \\
%  &
%   Lenet-5 &
%   12.117 &
%   1.215 &
%   0.768 &
%   1.047 &
%   2.125 &
%   6.303 \\
% \midrule
% \multirow{2}{*}{ImageNet} &
%   Densenet-161 &
%   5.721 &
%   0.744 &
%   2.014 &
%   4.723 &
%   3.103 &
%   6.575 \\
%  &
%   Resnet-152 &
%   6.544 &
%   0.791 &
%   1.985 &
%   5.805 &
%   3.528 &
%   4.977 \\
\midrule
SVHN &
  Resnet-152-SD &
  0.852 &
  0.552 &
  0.570 &
  0.573 &
  0.607 &
  \textbf{0.265} \\
\bottomrule
\end{tabular}
    \vspace{1ex}

    \caption{\em KS calibration error~\cite{gupta-spline-iclr21} (in \%) comparisons against state-of-the-art post-hoc calibration methods on image classification datasets: CIFAR-10 and SVHN, using various network architectures. Here, we use two dense g-layers with 32 units each for all our experiments.}
    \label{tab:res_PKSE}
    \vspace{-4ex}
\end{table*}


==> theorenv.tex <==
%
% Derived from article.sty and eccv92.sty
%

\catcode`\@=11

%
%
% New theorem environments
%
%
\newif\if@envcountreset\@envcountresetfalse
\def\ds@envcountreset{\@envcountresettrue}
\def\ts{\thinspace}
%
% new environments and theorems
% borrowed form the LTMP-style of Springer-Verlag
% designed by Dr. Christoph Ender
%
% define the new theorem like environments
% define a new style of environments where it is possible to define
% the font % used as the theorem name and the fontfamily for the text.
%
% \newstytheorem{name}{thefont}{txtfont}{Text}[Counter]
% \newstytheorem{name}{thefont}{txtfont}[oldname]{Text}
%
% #1 - name of theorem
% #2 - theorem font
% #3 - text font
%
\def\newstytheorem#1#2#3{%
\@ifnextchar[{\che@othm{#1}{#2}{#3}}{\che@nthm{#1}{#2}{#3}}}
%
% #1 - name of theorem
% #2 - theorem font
% #3 - text font
% #4 - text string of thorem name
%
\def\che@nthm#1#2#3#4{%
\@ifnextchar[{\che@xnthm{#1}{#2}{#3}{#4}}{\che@ynthm{#1}{#2}{#3}{#4}}}
%
% #1 - name of theorem
% #2 - theorem font
% #3 - text font
% #4 - text string of thorem name
% #5 - add theorem counter to reset list of another counter
%
\def\che@xnthm#1#2#3#4[#5]{\expandafter
\@ifdefinable\csname #1\endcsname
{\@definecounter{#1}\if@envcountreset\@addtoreset{#1}{#5}\fi
\expandafter\xdef\csname the#1\endcsname{\@thmcounter{#1}}%
\global\@namedef{#1}{\che@thm{#1}{#4}{#2}{#3}}\global
\@namedef{end#1}{\@endtheorem}}}
%
% #1 - name of theorem
% #2 - theorem font
% #3 - text font
% #4 - text string of thorem name
%
\def\che@ynthm#1#2#3#4{\expandafter\@ifdefinable\csname #1\endcsname
{\@definecounter{#1}%
\expandafter\xdef\csname the#1\endcsname{\@thmcounter{#1}}%
\global\@namedef{#1}{\che@thm{#1}{#2}{#3}{#4}}\global
\@namedef{end#1}{\@endtheorem}}}
%
% change oldthm if oldname in specification is '*'
% then don't use a counter
% #1 - countername
% #2 - theorem font
% #3 - text font
% #4 - counter used
% #5 - string containing theorem name to print
%
\def\che@othm#1#2#3[#4]#5{\expandafter\@ifdefinable
\csname#1\endcsname%
{\@@othm@{#1}{#2}{#3}{#4}{#5}\global\@namedef{end#1}{\@endtheorem}}}
%
\def\@@othm@#1#2#3#4#5{\if *#4{\global\@namedef{the#1}{\relax}
\global\@namedef{#1}{\@bthm@{}{#5}{#2}{#3}}}\else
{\global\@namedef{the#1}{\@nameuse{the#4}}% define the counter
\global\@namedef{#1}{\che@thm{#4}{#5}{#2}{#3}}}\fi}
%
% new defs for theorem environment che 17-MAR-1989
% it improves the option possible
%
% #1 - countername  = theorem name
% #2 - string containing theorem name to print
% #3 - theorem font
% #4 - text font
\def\che@thm#1#2#3#4{\@ifnextchar({\@athm{#1}{#2}{#3}{#4}}{%
\@ifnextchar *{\@bthm{#1}{#2}{#3}{#4}}%
{\@@thm{#1}{#2}{#3}{#4}}}}
%
% \begin{thm}(A.1)[test]      results in:
% \end{thm}                               thm A.1 (test) ....
% #1 - theorem
% #2 - string of theorem name
% #3 - font for theorem name and label
% #4 - Text font
% #5 - is the new label
% #6 - optional string
%
\def\@athm#1#2#3#4(#5){\@ifnextchar[{%
\@aythm{#1}{#2}{#3}{#4}{#5}}{\@axthm{#1}{#2}{#3}{#4}{#5}}}
\def\@axthm#1#2#3#4#5{\@@locthmlab{#1}{#5}%
\@begintheorem{#2}{#5}{#3}{#4}\ignorespaces}
\def\@aythm#1#2#3#4#5[#6]{\@@locthmlab{#1}{#5}%
\fuh@opargbegintheorem{#2}{#5}{#6}{#3}{#4}\ignorespaces}
%
% \begin{thm}*[xytest]        results in:
% \end{thm}                               thm (xytest) ....
% #1 - theorem
% #2 - string of theorem name
% #3 - font for theorem name and label
% #4 - Text font
% #5 - optional string
%
\def\@bthm@#1#2#3#4{\@ifnextchar[{\@bythm{#1}{#2}{#3}{#4}}{%
\@bxthm{#1}{#2}{#3}{#4}}}
\def\@bthm#1#2#3#4*{\@ifnextchar[{\@bythm{#1}{#2}{#3}{#4}}{%
\@bxthm{#1}{#2}{#3}{#4}}}
\def\@bxthm#1#2#3#4{\if !#1!\relax\else\@@locthmlab{#1}{}\fi
\@@begintheorem{#2}{#3}{#4}\ignorespaces}
\def\@bythm#1#2#3#4[#5]{%
\@@opargbegintheorem{#2}{#3}{#4}{#5}\ignorespaces}
%
% define local label
%   if no number or a user specified label occured
%
\def\@@locthmlab#1#2{\expandafter\def\csname the#1\endcsname{#2}
\let\@chetempa\protect\def\protect{\noexpand\protect\noexpand}%
\edef\@currentlabel{\csname p@#1\endcsname\csname the#1\endcsname}%
\let\protect\@chetempa}
%
% #1 - counter = theorem name
% #2 - string with name
% #3 - font for theorem name and label
% #4 - font for text
\def\@@thm#1#2#3#4{\refstepcounter
    {#1}\@ifnextchar[{\che@ythm{#1}{#2}{#3}{#4}}{%
    \che@xthm{#1}{#2}{#3}{#4}}}
%
\def\che@xthm#1#2#3#4{\che@begintheorem{#2}{\csname
the#1\endcsname}{#3}{#4}\ignorespaces}
\def\che@ythm#1#2#3#4[#5]{\che@opargbegintheorem{#2}{\csname
       the#1\endcsname}{#5}{#3}{#4}\ignorespaces}
%
% #1 - name of theorem
% #2 - label string
% #3 - font for name and lable
% #4 - text fomt
%
\def\che@begintheorem#1#2#3#4{#4\trivlist\item[#3 #1\ts #2.]}
%
% #1 - name of theorem
% #2 - label string
% #3 - additonal text
% #4 - font for name and lable
% #5 - text fomt
%
\def\che@opargbegintheorem#1#2#3#4#5{#5 \trivlist
\item[#4 #1\ts #2\ #3.]}
%
\def\fuh@opargbegintheorem#1#2#3{\it \trivlist
      \item[\hskip \labelsep{\bf #1\ #2\ (#3).}]}
%
\def\@@begintheorem#1#2#3{#3\trivlist\item[#2 #1.]}
\def\@@opargbegintheorem#1#2#3#4{#3\trivlist\item[#2 #1 #4.]}
 
\newstytheorem{theorem}{\bf}{\it}{Theorem}[section]
\newstytheorem{conjecture}{\bf}{\it}{Conjecture}[section]
\newstytheorem{example}{\bf}{\rm}[theorem]{Example}
\newstytheorem{proposition}{\bf}{\it}[theorem]{Proposition}
\newstytheorem{corollary}{\bf}{\it}[theorem]{Corollary}
\newstytheorem{lemma}{\bf}{\it}[theorem]{Lemma}
\newstytheorem{proof}{\it}{\rm}[*]{Proof}
\newstytheorem{definition}{\bf}{\rm}[theorem]{Definition}
\newstytheorem{remark}{\it}{\rm}[*]{Remark}
\newstytheorem{exercise}{\it}{\rm}[theorem]{Exercise}
\newstytheorem{problem}{\it}{\rm}[theorem]{Problem}
\newstytheorem{solution}{\it}{\rm}[theorem]{Solution}
\newstytheorem{note}{\it}{\rm}[theorem]{Note}
\newstytheorem{question}{\it}{\rm}[theorem]{Question}
\newstytheorem{condition}{\it}{\rm}[theorem]{Condition}
%\newstytheorem{algorithm}{\bf}{\rm}[theorem]{Algorithm}
\newstytheorem{numbered}{\bf}{\it}[theorem]{}
%\renewcommand{\thenumbered}{(\thesection.\arabic{numbered})}
\renewcommand{\thenumbered}{(\arabic{numbered})}
%\newstytheorem{unnumbered}{\bf}{\it}[*]{~~~$\bullet$\hspace*{-18pt}~~~} 
\newenvironment{unnumbered}{\begin{itemize}\item\em}{\end{itemize}}
%\renewcommand{\thetheorem}{\thesection.\arabic{theorem}}
\renewcommand{\thetheorem}{\arabic{theorem}}
 
% qed sign
\def\squareforqed{\hbox{\rlap{$\sqcap$}$\sqcup$}}
\def\qed{\ifmmode\squareforqed\else{\unskip\nobreak\hfil
\penalty50\hskip1em\null\nobreak\hfil\squareforqed
\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}

\catcode`\@=12

%\newstytheorem{unnumbered}{\bf}{\it}[*]{~~~$\bullet$\hspace*{-18pt}~~~} 
%\renewcommand{\thenumbered}{(\thechapter.\arabic{numbered})}


